Efficient Path-Sensitive Data-Dependence Analysis

This paper presents a scalable path- and context-sensitive data-dependence analysis. The key is to address the aliasing-path-explosion problem via a sparse, demand-driven, and fused approach that piggybacks the computation of pointer information with the resolution of data dependence. Specifically, our approach decomposes the computational efforts of disjunctive reasoning into 1) a context- and semi-path-sensitive analysis that concisely summarizes data dependence as the symbolic and storeless value-flow graphs, and 2) a demand-driven phase that resolves transitive data dependence over the graphs. We have applied the approach to two clients, namely thin slicing and value flow analysis. Using a suite of 16 programs ranging from 13 KLoC to 8 MLoC, we compare our techniques against a diverse group of state-of-the-art analyses, illustrating significant precision and scalability advantages of our approach.

==> Feedback.tex <==


The response on the novelty concern brings up some interesting points (related to the notion of sparsity and the filtering of paths in path-sensitive analyses). We think that these points should be discussed and evaluated further (but that means significant changes to the submission).

Reviewers were unsatisfied by the response on the lack of formalization. The paper should at least make the basic abstract predicates and analysis techniques clear. It should also clarify the soundness property guaranteed by this analysis design.

Overall, we found that the amount of changes to address these two points is too important, thus the paper should be rejected. We hope that our comments will help improve another version of this submission.

==> eval-alias-set.tex <==
\subsection{Thin Slicing Client}
\label{subsec:eval-slice}

We further compare \ToolName\ against \supa\ for thin slicing, which is introduced by~\citet{sridharan2007thin} to facilitate program  understanding and debugging.
A thin slice for a program variable, a.k.a., the slicing seed, includes only the \emph{producer statements} that directly affect the values of the variable.
In contrast to conventional slicing, control dependence and the data dependence of the variable's base pointer are excluded. Hence, thin slices are typically much smaller than conventional program slices. In this experiment, we generate thin slicing queries from the bug reports issued by a typestate analysis. 

%In what follows, we denote the slicers based on \supa\ and \ToolName\ as \supa-Slicer and \ToolName-Slicer, respectively. For each project, we randomly generate fifty thin slicing queries. 

Figure~\ref{eval:thin-slice} summarizes the results of this comparison. For each program, we report the average processing time and the average number of statements of each query. Note that we exclude the time for constructing data-dependence graphs in Figure \ref{eval:thin-slice}(a). The evaluation demonstrates that \ToolName\ is scalable for the thin slicing client, taking under 140 milliseconds for each demand query. As a summary, \ToolName\ is up to 302$\times$ faster than \supa, and 54$\times$ faster on average. Besides, the size of the slices produced by \ToolName\ is, on average smaller than \supa.  
Specifically, the average number of statements reported  by  \supa\ and \ToolName\ are 148 and 114, respectively.

The evaluation results indicate the improved precision of alias information, which is shown to be critical for the precision of thin slicing~\cite{sridharan2007thin,tripp2009taj}. An important reason is that \ToolName's quasi-path-sensitive analysis (\cref{subsec:pathupdate}) can prune away more spurious value flows than the demand-driven flow- and context-sensitive analysis based on \supa. 

\begin{figure*}[t]
	\centering
	\includegraphics[width=0.8\textwidth]{images/eval-slice}
	\caption{
		Comparing time cost and average slice sizes of \supa\ and \ToolName}
	\label{eval:thin-slice}
\end{figure*}


%%The alias set of a given pointer $p$ consists of all pointers that may alias with $p$. Alias set information is useful for applications that track the global information flow such as taint and typestate analyses ~\cite{naeem2009efficient,naeem2011faster,spath2017ide,spath2016boomerang}.  

%For the thin slicing client, we do not invoke an SMT solver to achieve full path-sensitivity, because the goal of thin slicing is to facilitate program  understanding and debugging, which typically requires fast response from the static analyzer.

%\textbf{Setup.} 
%In \ToolName, to query the alias set of a value $p$, we can perform a backward graph traversal from $p$ to collect the values $p'$ that can flow to $p$ and then proceed with a forward graph traversal to collect all values reachable from $v'$.  
%We configure \supa\ to answer demand-driven pointer queries with the precision of flow- and context-sensitivities, as described in~\cite{sui2016demand}. 

%For a fair comparison, we run \ToolName\ and \supa\ in single thread mode. 

==> fonts.tex <==
%----------------------------------------------------------
%-% Definition of fonts for Maths

%----------------------------------------------------------
%-% Math Bold fonts
\usepackage[bbgreekl]{mathbbol}
\newcommand{\mathboldcommand}[1]{\mathbb{#1}}
\newcommand{\bbA}{\mathboldcommand{A}}
\newcommand{\bbB}{\mathboldcommand{B}}
\newcommand{\bbC}{\mathboldcommand{C}}
\newcommand{\bbD}{\mathboldcommand{D}}
\newcommand{\bbE}{\mathboldcommand{E}}
\newcommand{\bbF}{\mathboldcommand{F}}
\newcommand{\bbG}{\mathboldcommand{G}}
\newcommand{\bbH}{\mathboldcommand{H}}
\newcommand{\bbI}{\mathboldcommand{I}}
\newcommand{\bbJ}{\mathboldcommand{J}}
\newcommand{\bbK}{\mathboldcommand{K}}
\newcommand{\bbL}{\mathboldcommand{L}}
\newcommand{\bbM}{\mathboldcommand{M}}
\newcommand{\bbN}{\mathboldcommand{N}}
\newcommand{\bbO}{\mathboldcommand{O}}
\newcommand{\bbP}{\mathboldcommand{P}}
\newcommand{\bbQ}{\mathboldcommand{Q}}
\newcommand{\bbR}{\mathboldcommand{R}}
\newcommand{\bbS}{\mathboldcommand{S}}
\newcommand{\bbT}{\mathboldcommand{T}}
\newcommand{\bbU}{\mathboldcommand{U}}
\newcommand{\bbV}{\mathboldcommand{V}}
\newcommand{\bbW}{\mathboldcommand{W}}
\newcommand{\bbX}{\mathboldcommand{X}}
\newcommand{\bbY}{\mathboldcommand{Y}}
\newcommand{\bbZ}{\mathboldcommand{Z}}
\newcommand{\bba}{\mathboldcommand{a}}
\newcommand{\bbb}{\mathboldcommand{b}}
\newcommand{\bbc}{\mathboldcommand{c}}
\newcommand{\bbd}{\mathboldcommand{d}}
\newcommand{\bbe}{\mathboldcommand{e}}
\newcommand{\bbf}{\mathboldcommand{f}}
\newcommand{\bbg}{\mathboldcommand{g}}
\newcommand{\bbh}{\mathboldcommand{h}}
\newcommand{\bbi}{\mathboldcommand{i}}
\newcommand{\bbj}{\mathboldcommand{j}}
\newcommand{\bbk}{\mathboldcommand{k}}
\newcommand{\bbl}{\mathboldcommand{l}}
\newcommand{\bbm}{\mathboldcommand{m}}
\newcommand{\bbn}{\mathboldcommand{n}}
\newcommand{\bbo}{\mathboldcommand{o}}
\newcommand{\bbp}{\mathboldcommand{p}}
\newcommand{\bbq}{\mathboldcommand{q}}
\newcommand{\bbr}{\mathboldcommand{r}}
\newcommand{\bbs}{\mathboldcommand{s}}
\newcommand{\bbt}{\mathboldcommand{t}}
\newcommand{\bbu}{\mathboldcommand{u}}
\newcommand{\bbv}{\mathboldcommand{v}}
\newcommand{\bbw}{\mathboldcommand{w}}
\newcommand{\bbx}{\mathboldcommand{x}}
\newcommand{\bby}{\mathboldcommand{y}}
\newcommand{\bbz}{\mathboldcommand{z}}
\newcommand{\bbga}{\mathboldcommand{\bbalpha}}
\newcommand{\bbgb}{\mathboldcommand{\bbbeta}}
\newcommand{\bbgc}{\mathboldcommand{\bbgamma}}
\newcommand{\bbgd}{\mathboldcommand{\bbdelta}}
\newcommand{\bbge}{\mathboldcommand{\bbepsilon}}
\newcommand{\bbgi}{\mathboldcommand{\bbiota}}
\newcommand{\bbgt}{\mathboldcommand{\bbtau}}
\newcommand{\bblbracket}{\mathboldcommand{\Lbrack}}
\newcommand{\bbrbracket}{\mathboldcommand{\Rbrack}}
\newcommand{\bblparen}{\llparenthesis}
\newcommand{\bbrparen}{\rrparenthesis}
\newcommand{\bblangle}{\mathboldcommand{\Langle}}
\newcommand{\bbrangle}{\mathboldcommand{\Rangle}}
\newcommand{\bblbrace}{\mathboldcommand{\{}} % KO
\newcommand{\bbrbrace}{\mathboldcommand{\}}} % KO
%----------------------------------------------------------

%----------------------------------------------------------
%-% Math caligraphic characters
\usepackage{euscript}
\newcommand{\mathcalcommand}[1]{\mathcal{#1}}
\newcommand{\mcA}{\mathcalcommand{A}}
\newcommand{\mcB}{\mathcalcommand{B}}
\newcommand{\mcC}{\mathcalcommand{C}}
\newcommand{\mcD}{\mathcalcommand{D}}
\newcommand{\mcE}{\mathcalcommand{E}}
\newcommand{\mcF}{\mathcalcommand{F}}
\newcommand{\mcG}{\mathcalcommand{G}}
\newcommand{\mcH}{\mathcalcommand{H}}
\newcommand{\mcI}{\mathcalcommand{I}}
\newcommand{\mcJ}{\mathcalcommand{J}}
\newcommand{\mcK}{\mathcalcommand{K}}
\newcommand{\mcL}{\mathcalcommand{L}}
\newcommand{\mcM}{\mathcalcommand{M}}
\newcommand{\mcN}{\mathcalcommand{N}}
\newcommand{\mcO}{\mathcalcommand{O}}
\newcommand{\mcP}{\mathcalcommand{P}}
\newcommand{\mcQ}{\mathcalcommand{Q}}
\newcommand{\mcR}{\mathcalcommand{R}}
\newcommand{\mcS}{\mathcalcommand{S}}
\newcommand{\mcT}{\mathcalcommand{T}}
\newcommand{\mcU}{\mathcalcommand{U}}
\newcommand{\mcV}{\mathcalcommand{V}}
\newcommand{\mcW}{\mathcalcommand{W}}
\newcommand{\mcX}{\mathcalcommand{X}}
\newcommand{\mcY}{\mathcalcommand{Y}}
\newcommand{\mcZ}{\mathcalcommand{Z}}
%----------------------------------------------------------

%----------------------------------------------------------
%-% Math Zaph Chancery characters
\DeclareMathAlphabet{\mathpzc}{T1}{pzc}{m}{it}
\newcommand{\zaphcommand}[1]{\mathpzc{#1}}
\newcommand{\bigzaphcommand}[1]{
  \text{\fontsize{14}{10}\usefont{T1}{pzc}{m}{it}{#1}}}
%\newcommand{\zaphcommand}[1]{
%  \text{\fontsize{11}{10}\usefont{T1}{pzc}{m}{it}{#1}}}
\newcommand{\zcA}{\zaphcommand{A}}
\newcommand{\zcB}{\zaphcommand{B}}
\newcommand{\zcC}{\zaphcommand{C}}
\newcommand{\zcD}{\zaphcommand{D}}
\newcommand{\zcE}{\zaphcommand{E}}
\newcommand{\zcF}{\zaphcommand{F}}
\newcommand{\zcG}{\zaphcommand{G}}
\newcommand{\zcH}{\zaphcommand{H}}
\newcommand{\zcI}{\zaphcommand{I}}
\newcommand{\zcJ}{\zaphcommand{J}}
\newcommand{\zcK}{\zaphcommand{K}}
\newcommand{\zcL}{\zaphcommand{L}}
\newcommand{\zcM}{\zaphcommand{M}}
\newcommand{\zcN}{\zaphcommand{N}}
\newcommand{\zcO}{\zaphcommand{O}}
\newcommand{\zcP}{\zaphcommand{P}}
\newcommand{\zcQ}{\zaphcommand{Q}}
\newcommand{\zcR}{\zaphcommand{R}}
\newcommand{\zcS}{\zaphcommand{S}}
\newcommand{\zcT}{\zaphcommand{T}}
\newcommand{\zcU}{\zaphcommand{U}}
\newcommand{\zcV}{\zaphcommand{V}}
\newcommand{\zcW}{\zaphcommand{W}}
\newcommand{\zcX}{\zaphcommand{X}}
\newcommand{\zcY}{\zaphcommand{Y}}
\newcommand{\zcZ}{\zaphcommand{Z}}
\newcommand{\zca}{\zaphcommand{a}}
\newcommand{\zcb}{\zaphcommand{b}}
\newcommand{\zcc}{\zaphcommand{c}}
\newcommand{\zcd}{\zaphcommand{d}}
\newcommand{\zce}{\zaphcommand{e}}
\newcommand{\zcf}{\zaphcommand{f}}
\newcommand{\zcg}{\zaphcommand{g}}
\newcommand{\zch}{\zaphcommand{h}}
\newcommand{\zci}{\zaphcommand{i}}
\newcommand{\zcj}{\zaphcommand{j}}
\newcommand{\zck}{\zaphcommand{k}}
\newcommand{\zcl}{\zaphcommand{l}}
\newcommand{\zcm}{\zaphcommand{m}}
\newcommand{\zcn}{\zaphcommand{n}}
\newcommand{\zco}{\zaphcommand{o}}
\newcommand{\zcp}{\zaphcommand{p}}
\newcommand{\zcq}{\zaphcommand{q}}
\newcommand{\zcr}{\zaphcommand{r}}
\newcommand{\zcs}{s}
\newcommand{\zct}{\zaphcommand{t}}
\newcommand{\zcu}{\zaphcommand{u}}
\newcommand{\zcv}{\zaphcommand{v}}
\newcommand{\zcw}{\zaphcommand{w}}
\newcommand{\zcx}{\zaphcommand{x}}
\newcommand{\zcy}{\zaphcommand{y}}
\newcommand{\zcz}{\zaphcommand{z}}
\newcommand{\bzcd}{\bigzaphcommand{d}}
%----------------------------------------------------------

%----------------------------------------------------------
%-% Math Fraktur fonts
%\usepackage{eufrak}
\newcommand{\mathfrakcommand}[1]{\mathfrak{#1}}
\newcommand{\fkA}{\mathfrakcommand{A}}
\newcommand{\fkB}{\mathfrakcommand{B}}
\newcommand{\fkC}{\mathfrakcommand{C}}
\newcommand{\fkD}{\mathfrakcommand{D}}
\newcommand{\fkE}{\mathfrakcommand{E}}
\newcommand{\fkF}{\mathfrakcommand{F}}
\newcommand{\fkG}{\mathfrakcommand{G}}
\newcommand{\fkH}{\mathfrakcommand{H}}
\newcommand{\fkI}{\mathfrakcommand{I}}
\newcommand{\fkJ}{\mathfrakcommand{J}}
\newcommand{\fkK}{\mathfrakcommand{K}}
\newcommand{\fkL}{\mathfrakcommand{L}}
\newcommand{\fkM}{\mathfrakcommand{M}}
\newcommand{\fkN}{\mathfrakcommand{N}}
\newcommand{\fkO}{\mathfrakcommand{O}}
\newcommand{\fkP}{\mathfrakcommand{P}}
\newcommand{\fkQ}{\mathfrakcommand{Q}}
\newcommand{\fkR}{\mathfrakcommand{R}}
\newcommand{\fkS}{\mathfrakcommand{S}}
\newcommand{\fkT}{\mathfrakcommand{T}}
\newcommand{\fkU}{\mathfrakcommand{U}}
\newcommand{\fkV}{\mathfrakcommand{V}}
\newcommand{\fkW}{\mathfrakcommand{W}}
\newcommand{\fkX}{\mathfrakcommand{X}}
\newcommand{\fkY}{\mathfrakcommand{Y}}
\newcommand{\fkZ}{\mathfrakcommand{Z}}
\newcommand{\fka}{\mathfrakcommand{a}}
\newcommand{\fkb}{\mathfrakcommand{b}}
\newcommand{\fkc}{\mathfrakcommand{c}}
\newcommand{\fkd}{\mathfrakcommand{d}}
\newcommand{\fke}{\mathfrakcommand{e}}
\newcommand{\fkf}{\mathfrakcommand{f}}
\newcommand{\fkg}{\mathfrakcommand{g}}
\newcommand{\fkh}{\mathfrakcommand{h}}
\newcommand{\fki}{\mathfrakcommand{i}}
\newcommand{\fkj}{\mathfrakcommand{j}}
\newcommand{\fkk}{\mathfrakcommand{k}}
\newcommand{\fkl}{\mathfrakcommand{l}}
\newcommand{\fkm}{\mathfrakcommand{m}}
\newcommand{\fkn}{\mathfrakcommand{n}}
\newcommand{\fko}{\mathfrakcommand{o}}
\newcommand{\fkp}{\mathfrakcommand{p}}
\newcommand{\fkq}{\mathfrakcommand{q}}
\newcommand{\fkr}{\mathfrakcommand{r}}
\newcommand{\fks}{\mathfrakcommand{s}}
\newcommand{\fkt}{\mathfrakcommand{t}}
\newcommand{\fku}{\mathfrakcommand{u}}
\newcommand{\fkv}{\mathfrakcommand{v}}
\newcommand{\fkw}{\mathfrakcommand{w}}
\newcommand{\fkx}{\mathfrakcommand{x}}
\newcommand{\fky}{\mathfrakcommand{y}}
\newcommand{\fkz}{\mathfrakcommand{z}}


==> inter-long.tex <==
\section{Detailed}


\subsection{Parameterized Summary}

To achieve context-sensitivity, conventional summary-based analyses
conservatively identify the side effects of a function,
which are then cloned at every call site of the summarized function in the upper-level callers~\cite{xie2005scalable,dillig2011precise}.  
However, the size of the side-effect summary can quickly explode and become a significant obstacle to scalability. To illustrate, consider the program in Figure~\ref{ptgraph-clone}(a).
In conventional approaches, the summary of \textit{foo} is the points-to information, $\mathbb{E}$ and $\mathbb{S}$, of the interface variable $y$ at the exit point of \textit{foo}. That is,
$$
\mathbb{E}(y) = \{ (\texttt{true}, o) \}; \enskip
\mathbb{S}(o) = \{ (\varphi, \ell_1, a),  (\neg \varphi, \ell_2, b) \};
$$
By cloning the summary to the two call sites in \textit{qux} and \textit{bar},
the two variables $a$ and $b$ are cloned twice.
When the summaries of \textit{qux} and \textit{bar} are cloned to their upper-level callers, $a$ and $b$ will continue to be cloned. As a result, the summary size will grow exponentially.

To mitigate the problem, our basic idea is to introduce auxiliary variables, each of which stands for a class of variables to clone.
Then we can only clone a single auxiliary variable during interprocedural analysis to reduce the burden of cloning.
For the above example, we introduce an extra value $R$ for the function \textit{foo} to represent all values (e.g., $a$ and $b$) stored in the memory object pointed-to by $y$.
As a result, 
the function summary gets smaller as the following, and we only need to clone a single variable $R$ to the callers at the time of interprocedural analysis. 
\begin{align*}
\begin{split}
\mathbb{E}(y)  &=  \{ (\texttt{true}, o) \}; \\
\mathbb{S}(o)   &= \{ (\texttt{true}, \ell_3, R) \};  \\
R               &\mapsto \{ (\varphi, \ell_1, a),  (\neg \varphi, \ell_2, b) \} \\ 
\end{split}
\end{align*}

Intuitively, this process is amounts to adding an extra return value to the function \textit{foo}, as shown in Figure~\ref{ptgraph-clone}(b). Formally, this summarization process is illustrated in Algorithm~\ref{aux-summary2}, where the points-to results are always merged into a single auxiliary variable so that the burden of the cloning processes can be reduced. Intuitively, each auxiliary variable stands for a modified non-local memory object accessed through an access path\footnote{An access path refers to a combination of dereferencing and field access operations~\cite{deutsch1992storeless,kanvar2016heap}.} rooted at an interface variable.

\begin{algorithm}[t]
	\caption{Summarize an interface variable}
	\label{aux-summary2}
	\KwIn{An interface variable (parameter or return) $x$}
	\KwOut{Updated $\mathbb{E}, \mathbb{S}$ with auxiliary variables}
	%\DontPrintSemicolon
	
	$WL \leftarrow \{ x\}$\;
	\While{$WL$ is not empty} {
		$x \leftarrow$ pop an element from $WL$\;
		$R, o_x \leftarrow $ create an auxiliary variable and a memory object\;
		\For{$(\pi, o) \in  \mathbb{E}(x)$} {	
			%$V_o \leftarrow $ an auxiliary variable\;
			\For{$(\varphi, \ell', v) \in \Pi_{\pi}(\mathbb{S}(o))$}{
				%$V_o \leftarrow V_o \cup \{(\varphi, \ell', v)\}$ \;	
				$\mathbb{E}(R) \leftarrow \mathbb{E}(R) \cup \Pi_{\varphi}(\mathbb{E}(v))$ \;	
			}
			%$\mathbb{S}(o) \leftarrow \mathbb{S}(o) \cup \{ (\pi, \ell, V_o) \}$ \;
			%$R \leftarrow R \cup V_o$\;
		}
		$\mathbb{E}(x) \leftarrow \{ (\texttt{true}, o_x) \}$,
		$\mathbb{S}(o_x) \leftarrow \{ (\texttt{true}, \_, R) \}$\;
		%Insert a store staement $\ell: R = *x$\;
		\If{$R$ is a pointer}{ $WL \leftarrow WL \cup \{ R\}$}
	}   
\end{algorithm}

\smallskip

%\textbf{Summary Application.} At a high level, when a caller may invoke a summarized function $f$, we apply the summary of $f$ instead of cloning its full body at the call site, as shown with the rules in Figure \ref{inter-rules}.  For simplicity of presentation, suppose we have that $AP(F) = AP(R) = *z$, where $z, F, R$ are the formal parameter, aux-parameter, and aux-return value of $f$, respectively. 
%
%Rule \textsc{InstSymbol} first creates the symbolic variables $A, L$ in the caller, which serve as the ``clones'' of  $F, R$, respectively. Then it instantiates the context-specific mapping of $f$'s  parameters to actuals, denoted by $\mathbb{M}$. The mapping of formal parameters is straightforward, and hence, we focus on the aux-parameters. Suppose we have $\mathbb{M}(z) = \{ (\texttt{true}, \ell, u) \}$, then we can instantiate $F$ by querying the values that can be loaded from $*u$. Besides, rule \textsc{InstSymbol} updates the abstract store by recording that $L$ is stored into the memory objects pointed by $u$.
%
%
%\begin{figure*}[t]	
%	{\centering
%		\[
%		\inference[\textsc{InstSymbol}($\ell, \psi: \textit{call} \ \  f(u), F, R$)]
%		{
%			\mathbb{M}(z) = \{ (\texttt{true}, \ell, u) \}, A = F, L = R, \\
%			\forall(\pi, o) \in \Pi_{\psi}(\mathbb{E}(u)), \\
%			\forall(\varphi, \ell', g) \in \Pi_{\pi}(\mathbb{S}(o)) \\
%		}
%		{
%			\mathbb{M}'(F) = \mathbb{M}(F) \cup \{ (\varphi, \ell', g) \}, \mathbb{S'}(o) = \mathbb{S}(o) \cup \{ (\pi, \ell, L) \}
%		}
%		\]
%		
%		\[
%		\inference[\textsc{LinkValue}($\ell, \psi: \textit{call} \ \  f(u), F, R$)]
%		{
%			p \in Val(R) \text{ a parameter}, \\
%			\forall (\varphi, \ell', g) \in \mathbb{M}(p)
%		}
%		{
%			\mathbb{E}'(L) = \mathbb{E}(L) \cup \Pi_{\psi}(\mathbb{E}(g))
%		}
%		\]
%		
%		\[
%		\inference[\textsc{CloneObj}($\ell, \psi: \textit{call} \ \  f(u), F, R$)]
%		{
%			p \in Val(R) \text{  points-to an allocation site in } f\\
%		}
%		{
%			\mathbb{E}'(L) = \mathbb{E}(L) \cup clone\_obj(\mathbb{E}(p))
%		}
%		\]
%	}
%	\caption{Apply a callee summary for function $f(z)$  at a call site, where $AP(F) = AP(R) = *z$}	
%	\label{inter-rules}
%\end{figure*}
%
%Rule \textsc{LinkValue} and Rule \textsc{CloneObj} simulate the memory behaviors of the function call with the symbolic summary.  Notice that $R$ can be data-dependent on a formal or aux-parameter, whose values are already encoded in $\mathbb{M}$ after applying the aforementioned \textsc{InstSymbol} rule. Hence, we can update the points-to environment $\mathbb{E}(L)$ by tracking the values on which $L$ is data-dependent.  Also, if a memory object allocated at the callee and its address can flow to $R$, rule \textsc{CloneObj} will clone the escaped object to distinguish allocations made at different call sites~\cite{MoPPA,lattner2007making}. 

%Figure xx shows and example, which ...

%We noticed that the IFDS/IDE approaches solve this problem much more efficiently, in which the summary edges
%are built after analyzing each function, transferring the input
%data flow facts to the output without re-analyzing the function. These input-to-output fast tracks are used on-demand to
%the relevant data-flow problems and, therefore, avoid blindly
%inlining the unused data flow results to the callers.


\subsection{On-Demand Search}
Alongside the analysis, we have been able to construct the local data-dependence graph (\cref{sec:domain}) for each function. The graph has two types of edges representing data-dependence relations: the \emph{direct edge} connects a store to a load  using the rule in Figure ~\ref{vfrule},  whereas the \emph{summary edge} connects $s$ to $t$ if $t$ is transitively data-dependent on $s$. The analysis eagerly connects the summary edges 
between a formal argument (formal-in) at the function entry and the return value (formal-out) at the function
exit. Such edges can be used at call sites to compute the dependence statements of the caller without going through the callee's function body.
%Summary edges between other types of values, e.g., from a parameter to a source/sink, are obtained on demand when checking certain kinds of properties.

\yao{I summarize some benefits}

With the local data-dependence graphs in hand, the client analysis can track data-dependence relations for variables of interest in a demand-driven fashion when checking source-sink properties, during which the alias constraints and  property-specific constraints are stitched together. 
Our design has two advantages.
First, it enhances precision, as a combined domain of pointer and source-sink information allows more precise information than could be obtained by solving each domain separately~\cite{Cousot:1979:SDP:567752.567778}. Second, it allows scalability, because the client analysis can dynamically (during property checking)
make distinctions between objects that the underlying pointer analysis
does not distinguish when constructing the data-dependence graphs.
Hence, the client concentrates computational effort on context- and path-sensitive pointer information only where it matters to the properties of interest.

%the local data-dependence graphs are stitched together by matching formal and actual parameters as well as return value and its receivers.  

As an example, consider the program in Figure~\ref{ptgraph-clone}(a). The data-dependence graphs of \textit{foo} and \textit{bar} are shown in Figure~\ref{ptgraph-clone}(c). Suppose we need determine if $n$ aliases with $a$. We traverse data-dependence graphs starting  from $a$ and obtain one complete  path from $a$ to $n$. We then solve the gathered path condition $\varphi$. To wit, the interprocedurally path-sensitive computations are only carried out for variables of interests. 

\smallskip
\textbf{Summary.} To achieve context-sensitivity but avoid expensive summary cloning,
we only clone the access-paths that are rooted at function parameters and incur side-effects, thus avoiding computing a whole-program image of the heap. 
The concise summary enables local reasoning of the data dependence, as opposed to global reasoning about the entire heap. 
The clones serve as context-sensitive ``conduits'' to allow values of interests flow in and out of the function scope on demand when checking source-sink properties.




==> related-context.tex <==
\subsection{Context-sensitive Pointer Analysis}
\label{subsec:related-ctx}

Existing context-sensitive pointer analyses 
are either clone-based \cite{whaley2004cloning, milanova2002parameterized,zhu2004symbolic,bravenboer2009strictly} or summary-based \cite{wilson1995efficient,whaley1999compositional,Ryder-RCI,nystrom2004bottom,yu2010level,dillig2011precise,li2013precise,sui2014making}, or CFL-reachability based \cite{sridharan2006refinement,xu2009scaling,shang2012demand,lu2013incremental}. 
%There is no consensus on the best solution.

\citet{wilson1995efficient} present a context-sensitive based on partial transfer functions (PTF) as function summaries. The work sparks a line of pointer analyses that are intra-procedurally flow-sensitive and generate function summaries to be instantiated at call sites.

%There are two styles of summary-based approaches that capture the aggregate effect of aliasing between function parameters: relevant context inference (RCI) \cite{Ryder-RCI} and partial transfer function (PTF) \cite{wilson1995efficient}. RCI constructs one transfer function  eagerly by assuming the presence of all possible entry aliasing, while PTF builds multiple transfer functions lazily based on different aliasing at its callsites. PTF requires reanalysis of function.

==> related-long.tex <==
\section{Related work}
We will discuss related work from six dimensions:
\begin{enumerate}
	\item Sparse analysis
	\item Path-sensitive analysis
	\item Demand-driven analysis
	\item Hybrid analysis
	\item Parallel analysis
	\item Other solutions of aliasing
\end{enumerate}

\subsection{Sparse pointer analysis}
%Many flow-sensitive analyses exploit  some form of sparsity to improve efficiencies, where def-use chains are captured by various sparse representation such as partial SSA \cite{cytron1989efficient} and sparse evaluation graphs \cite{choi1991automatic}.
\citet{hardekopf2009semi} present an inclusion-based, \emph{semi-sparse} flow-sensitive pointer analysis by leveraging the partial SSA IR \cite{lattner2004llvm} in LLVM.  Yet, the algorithm is sparse only on top-level variables, whose def-use chains are already available in the IR. 

To be fully sparse, a pointer analysis needs the def-use information of address-taken variables, which also requires reasoning about aliasing. To address this issue, there are two classes of full-sparse analysis.
\begin{enumerate}
	\item \emph{Staged sparse analysis} \cite{hardekopf2011flow,sui2016sparse, sui2016demand,yan2018spatio} exploits def-use chains pre-computed by a whole-program and exhaustive pre-analysis \footnote{(The def-use information of address-taken variables is encoded in the forms of memory SSA or value flow graph) }. Most existing methods use a flow- and context- insensitive Andersen analysis as the pre-analysis. There are two limits:
	\begin{enumerate}
		\item The imprecise pre-analysis introduces spurious value flows that can be performance-detrimental.
		\item The pre-analysis itself might be time-consuming for large-scale programs \cite{hardekopf2007ant}.
	\end{enumerate}
	\item \emph{On-the-fly sparse analysis} constructs a spare representation alongside the pointer analysis.  Existing solutions \cite{chase1990analysis, yu2010level,sui2011spas,li2011boosting} are  exhaustive and can be notoriously expensive. 
\end{enumerate} 

Why are existing on-they-fly sparse analyses exhaustive? \texttt{LevPA} \cite{yu2010level} and \texttt{SPAS} \cite{sui2011spas}'s idea is to run the analysis ``level-by-level''. They first perform Steensgaard's analysis to assign a \emph{level} to each pointer \footnote{Note that they do not use Steensgaard's analysis to build the memory SSA}, and then re-analyze the program level by level. They must be exhaustive for three reasons:
\begin{enumerate}
	\item A single level can consist of pointers from the whole program; 
	\item Pointers with lower levels strictly depend on the results of pointers with higher levels;
	\item Pointers from a particular client can have different levels. 
\end{enumerate}
Similarly, the analysis in \cite{li2011boosting} relies on an \emph{escape order} of pointers. The   order is not complete until all pointers are analyzed. 

\paragraph{Our work} We follow the ``on-the-fly sparse'' methodology. The crux is to obviate the requirement of an exhaustive analysis \cite{chase1990analysis, yu2010level,sui2011spas}. Our key observation is that we can determine data dependencies without deriving the full points-to sets. Therefore, we adopt a \emph{whole-program-points}, \emph{lazy} pointer analysis, which is sufficient to compute precise dependence edges, alleviating the need of eagerly incorporating pointer information.


\subsection{Path-sensitive pointer analysis} 
\paragraph{Challenges}  
The difficulty comes from the sheer number of constraints to handle. In path-sensitive pointer analysis,  a constraint is the Boolean combinations of constraints associated with existing pointer facts. Two factors can  quickly cause the explosion of constraints:
\begin{enumerate}
	\item When analyzing a single instruction, such as $p = *x$,  we may need to solve a large number of constraints, subject to the number of locations pointed by $x$ (i.e., $ | pts(x) |$);
	\item A function can have hundreds of thousands of pointer instructions. 
\end{enumerate}
The explosion is independent of (but compounded by) the problem of path-explosion caused by conditional branching in symbolic execution. 


\paragraph{Path abstraction}
Path-sensitivity comes in many flavors, depending on the kind of path information encoded as constraints. 
\begin{itemize}
	\item SPAS \cite{sui2011spas} performs a relatively coarse abstraction, where Boolean formulas abstract just the control flow, ignoring the actual predicate of a condition.  
	
	For instance,  we use two independent Boolean variables $b_1, b_2$ to mark the branches, not matter what \texttt{b1}, \texttt{b2} are.
	  \begin{verbatim}
	    foo() {
	      if (b1) {}  // b1: x == 2
	      if (b2) {}  // b2: x != 2
	    }
	  \end{verbatim}
	
	\item Saturn \cite{hackett2006aliasing}  and Compass \cite{dillig2011precise} adopt much more expensive abstractions that track also data predicates. 
\end{itemize}
The guards in our approach are conceptually first-order formulas, but abstracted as \emph{Boolean skeleton}, similar to the DPLL($T$) SMT solving algorithm. For instance, we abstract the two branch conditions $x = 2$ and $x \neq 2$ as Boolean literals $p$ and $\neg p$, respectively. Such encoding allows for certain degrees of branch correlation tracking.

In addition, we adopt several \emph{sound and linear time} algorithms as semi-decision procedures to make the path-sensitive analysis tractable. %Disjunctive abstract interpretation such as \emph{track partition} \cite{mauborgne2005trace} and \emph{elaborations} \cite{sankaranarayanan2006static} can introduce a form of path-sensitivity, but also needs reason about path predicates to prune infeasible paths.

\paragraph{Benefits of path-sensitivity}
We highlight the benefits of path-sensitivity in pointer analysis, that give rise to improved precision over flow-sensitive analysis.
\begin{enumerate}
	\item \emph{Strong update}. Strong updates require the use of must-alias/must-points-to
	information. Similar to \cite{dillig2011precise}, our path-sensitive, fine-grained memory abstraction exposes more opportunities for performing strong updates at STORE.
	
	\item \emph{Beyond strong update}.  Traditional approaches \cite{hackett2006aliasing,dillig2011precise} only focus on the effects strong update at STORE,  but may miss correlations between different STORE and LOAD. 

	We propose to perform  ``\emph{relevant updates}'' at LOAD for tracking the correlations. Shortly speaking, even our analysis cannot kill all values at a STORE,  it may ``kill certain values for a specific LOAD'' by pruning unsatisfiable constraints.
\end{enumerate}



\paragraph{Summary} In summary, compared with existing work,
\begin{enumerate}
	\item We introduce the notion of  ``relevant updates'' for tracking path-correlations between STORE and LOAD. Strong updates and relevant updates translate into significant gains in both precision and performance, because smaller points-to sets lead to less work \cite{lhotak2008evaluating,smaragdakis2014introspective}.
	\item By leveraging the novel path abstraction and semi- decision procedures, we pay affordable overhead for potentially performing the updates.
\end{enumerate} 

\subsection{Demand-driven pointer analysis} 
Demand-driven methods typically start with a relatively imprecise abstraction and recover precision  through on-demand refinement. To date, most demand-driven pointer analyses are either
\begin{itemize}
	\item Flow- and context- insensitive \cite{heintze2001demand,sridharan2005demand,saha2005incremental,zheng2008demand, zhang2014efficient}, or 
	\item Flow-insensitive, context-sensitive  \cite{sridharan2006refinement, yan2011demand, shang2012demand,liang2011scaling,liang2011learning, feng2015explorer}
\end{itemize}
Unfortunately, on-demand flow- and/or path- sensitive analysis has received relatively little attention \cite{guyer2005error,spath2016boomerang,sui2016demand,yan2018spatio}. \citet{spath2016boomerang} present \texttt{Boomerang}, an IFDS-based, flow- and context-sensitive alias-set analysis that does not pre-compute points-to information. \texttt{SUPA} \cite{sui2016demand} is a demand-driven, flow- and context- sensitive sparse pointer analysis, which uses a pre-analysis to construct the value flow graph (VFG).

%To date, most existing demand-driven analyses either start with no points-to information resolved \cite{sridharan2006refinement,yan2011demand},  or only pre-compute a flow- and context- insensitive solution \cite{blackshear2013thresher,sui2016demand, feng2015explorer, yan2018spatio}.
Current analyses may incur intractable overhead to perform flow-, path-, and context- sensitive refinement (\citet{blackshear2013thresher,yan2018spatio}) for two reasons: 
\begin{enumerate}
	\item The initial abstraction can result in many false warnings in bug hunting. As the abstraction is frequently refined, scalability suffers.
	\item  The initial abstraction cannot boost the refinement procedure well.
	   \begin{enumerate}
	   	\item  The ``pointer expression graph'' in \cite{zheng2008demand, sridharan2006refinement} looses control flow information. We even cannot perform flow- and path- sensitive analysis on the graph.
	   	%\item  Flow- and context- insensitive initial abstraction: \citet{blackshear2013thresher}
	   	\item \citet{sui2016demand} and \citet{yan2018spatio} use a pre-analysis to construct the value flow graph (VFG) that enables a \emph{sparse} refinement. However, the imprecise pre-analysis blows up the VFG with false edges, which can be performance-detrimental.
	   \end{enumerate}
\end{enumerate}

\paragraph{Our work} Our analysis bears similarities to demand-driven approaches in that it decomposes the cost of fully path-sensitive data dependence analysis for bug hunting.  

The delicate balancing act is that we define a \emph{relatively precise and practical} initial abstraction, i.e. the symbolic expression graph (SEG):
\begin{enumerate}
	\item We flow- and path- sensitively resolve pointer dependencies inside a function in the fully sparse manner.
	\item We context-sensitively track value dependences across function boundaries without exhaustively propagating pointer information. More specifically, our analysis
	  \begin{itemize}
	  	\item only clones parameterized pointer interface summaries;
	  	\item does not clone non-pointer heap values (e.g., an integer field of a C structure )
	  \end{itemize}
\end{enumerate}

\subsection{Hybrid pointer analysis}
There is an increasing interest in \emph{hybrid analyses} \footnote{We do not refer to hybrid static and dynamic analysis} that resemble demand-driven approaches. However, hybrid analyses are not queries-/client- driven; they can schedule specific strategies for different kinds of pointers without knowing the client.

\citet{lhotak2011points} attempt to perform strong updates on flow-sensitive singleton objects but falls back to the flow-insensitive points-to information otherwise. \citet{dvanhorn:Kastrinis2013Hybrid} treats virtual and static method calls differently, attempting to emulate callsite-based context sensitivity (i.e., $k$-CFA) for static method calls and object-sensitivity for dynamic calls. \emph{Introspective analysis} \cite{smaragdakis2014introspective} tunes context sensitivity per-method based on a pre-analysis that compute heuristics such as ``total points-to information'' \footnote{Note that it is different from the \emph{staged sparse} flow-sensitive analysis, where the pre-analysis is used to build a memory SSA}. \cite{jeong2017data} present a data-driven approach to guiding context-sensitive analysis. It assigns each method an appropriate context length including zero (i.e., context insensitivity) based on 25 atomic features. 


Hybrid analyses can be beneficial to classes of clients \cite{smaragdakis2014introspective, jeong2017data,li2018scalability}. Nonetheless, two limitations are notable.
\begin{enumerate}
	\item \emph{Unneeded pointer information is computed}, because hybrid approaches are not aware of the needs of their clients. We believe that hybrid analysis could be combined with traditional demand-driven approaches.
	\item \emph{Precisions are sacrificed}, even for pointers from the same client. For example, \citet{jeong2017data} assign each  function an appropriate context length. An improperly scheduled function can lead to high false positives.
\end{enumerate}

\paragraph{Our work}
Similar to hybrid approaches, our analysis results can be transparently reused by different clients.
If considering only a particular client such as use-after-free detection,
\begin{enumerate}
	\item Our analysis may also compute unneeded pointer information in the SEG (symbolic expression graph) construction phase;
	\item However, we can achieve \emph{the same high precision for the relevant pointers}, because the relevant transitive data dependencies are resolved on demand in the bug hunting phase. 
\end{enumerate}



\subsection{Parallel pointer analysis}
\citet{Mathew2010Parallel} formulate Andersen's analysis in terms of graph rewiring rules. The algorithm is further implemented on GPUs \cite{M2012AGPU}.  D4 \cite{liu2018d4} introduces an incremental Andersen's analysis which is parallel within each iteration of fixed-point computation. \citet{Nagaraj2013Parallel} propose a flow-sensitive analysis based on the graph-rewriting rules in \cite{Mathew2010Parallel}. PSEGPT \cite{zhao2018parallel} is also a parallel flow-sensitive analysis but builds heap def-use chains on-the-fly. \citet{Su2014Parallel} introduce a demand-driven, context-sensitive analysis that runs CFL-reachability operations in parallel and focuses on inter-query parallelism. %\citet{Edvinsson2011Parallel} present a GPU-based implementation of control flow analysis for functional languages.

Our work is similar to \cite{Putta2012Parallel} and \cite{Edvinsson2011Parallel}:  each thread has its own copy of variables and associated points-to sets, and  the results are merged after several sub-threads have finished. The main differences include:  
\begin{enumerate}
	\item  Our analysis is sparse and demand-driven that does not compute full points-to sets
	\item They partition points-to constraints and run multi-threads to propagate
	points-to information, while our parallelization is function-level with less thread interleaving.  
\end{enumerate}
Saturn \cite{xie2005scalable} also supports function-level parallel analysis, but we are unable to find the evaluation results in \cite{hackett2006aliasing}.



==> related-valueflow.tex <==
\subsection{Value Flow Analysis}
\label{subsec:related-valueflow}

%The analysis of value flows has been studied in different contexts in the programming language community, such as reaching definitions~\cite{cytron1991efficiently,bodik1998path} in data flow analysis, control-flow analysis~\cite{jones1979flow,shivers1991control} of functional programming languages, and taint analysis~\cite{tripp2009taj,tripp2013andromeda,arzt2014flowdroid}. 
In this section, we discuss related work on value flow analysis for bug hunting. Most existing approaches~\cite{das2002esp,DorVF2004,fastcheck-07} rely on a path-insensitive points-to or alias analysis to approximate data dependence. The value flow analyses inherit the imprecision from the pointer analysis.  
%ESP~\cite{das2002esp,DorVF2004} uses an off-the-shelf context-sensitive flow-insensitive points-to analysis~\cite{Das:2001:EIS:647170.718301}. 


%Fastcheck~\cite{fastcheck-07} 


%Backward symbolic analyis:  ESC/Java, Snugglebug \cite{Snugglebug} perform backward symbolic analysis and employ online formulas simplifications to improve scalability.  PSE \cite{PSE}. \citet{snelting2006efficient}

%The notion of value flow has recently been leveraged in pointer analysis \cite{li2011boosting,li2013precise,sui2016demand,li2018scalability}.~\citet{li2011boosting} perform a flow-sensitive points-to analysis alongside the construction of a  value-flow graph. \citet{sui2016demand} leverage a pre-computed value-flow graph to enable a sparse demand-driven analysis.~\citet{li2018scalability} use the object-flow graph for automatic tuning of context-sensitivity.
                         

==> vfg.tex <==
\section{Different value flow graph}


\subsection{Store-based VFG}

\subsection{Storeless VFG}

\begin{itemize}
	\item \emph{Match edges} in \cite{sridharan2006refinement}. The edges from stored to loads are based solely on filed types, without
	checking whether they access a common object.
	\item The edges connecting a
	store to a load in TAJ \cite{tripp2009taj} is computed by a
	preliminary pointer analysis.
\end{itemize}




Parameter handling is made explicit by special vertices for formal and actual parameters which are connected by copy-in and copy-out edges.
